Susceptibility of Communities against Low-Credibility Content in Social News Websites

Social news websites, such as Reddit, have evolved into prominent platforms for sharing and discussing news. A key issue on social news websites sites is the formation of echo chambers, which often lead to the spread of highly biased or uncredible news. We develop a method to identify communities within a social news website that are prone to uncredible or highly biased news. We employ a user embedding pipeline that detects user communities based on their stances towards posts and news sources. We then project each community onto a credibility-bias space and analyze the distributional characteristics of each projected community to identify those that have a high risk of adopting beliefs with low credibility or high bias. This approach also enables the prediction of individual users' susceptibility to low credibility content, based on their community affiliation. Our experiments show that latent space clusters effectively indicate the credibility and bias levels of their users, with significant differences observed across clusters -- a $34\%$ difference in the users' susceptibility to low-credibility content and a $8.3\%$ difference in the users' susceptibility to high political bias.

==> abstract.tex <==
Social news websites, such as Reddit, have evolved into prominent platforms for sharing and discussing news. A key issue on social news websites sites is the formation of echo chambers, which often lead to the spread of highly biased or uncredible news. We develop a method to identify communities within a social news website that are prone to uncredible or highly biased news. We employ a user embedding pipeline that detects user communities based on their stances towards posts and news sources. We then project each community onto a credibility-bias space and analyze the distributional characteristics of each projected community to identify those that have a high risk of adopting beliefs with low credibility or high bias. This approach also enables the prediction of individual users' susceptibility to low credibility content, based on their community affiliation. Our experiments show that latent space clusters effectively indicate the credibility and bias levels of their users, with significant differences observed across clusters---a $34\%$ difference in the users' susceptibility to low-credibility content and a  $8.3\%$ difference in the users' susceptibility to high political bias.

% Social news websites, such as Reddit, have become standard media for sharing and discussing news content. Echo chambers are a driving cause of misinformation and extremist views on social news websites, often driving large communities of users to adopt highly biased or low-credibility views. We investigate which communities in a social news website are susceptible to high-bias or low-credibility content. Our method relies on a user embedding pipeline, that detects user communities based on the stances they hold against the posts and news sources. We then project these communities onto a credibility-bias space and analyze the distributional characteristics of each projected cluster to identify which clusters have a high risk of adopting beliefs with low credibility or high bias. This method allows us to predict each user's susceptibility to low-credibility content based on their community. Our results indicate that the latent space clusters are good indicators of credibility and bias of their users, with a three-fold percentage difference in the ratio of low-credibility users and a 23-fold ratio percentage in the ratio of high-bias users across all different clusters
